Deep orthogonal decomposition: a continuously adaptive data-driven approach to model order reduction

We develop a novel deep learning technique, termed Deep Orthogonal Decomposition (DOD), for dimensionality reduction and reduced order modeling of parameter dependent partial differential equations. The approach consists in the construction of a deep neural network model that approximates the solution manifold through a continuously adaptive local basis. In contrast to global methods, such as Principal Orthogonal Decomposition (POD), the adaptivity allows the DOD to overcome the Kolmogorov barrier, making the approach applicable to a wide spectrum of parametric problems. Furthermore, due to its hybrid linear-nonlinear nature, the DOD can accommodate both intrusive and nonintrusive techniques, providing highly interpretable latent representations and tighter control on error propagation. For this reason, the proposed approach stands out as a valuable alternative to other nonlinear techniques, such as deep autoencoders. The methodology is discussed both theoretically and practically, evaluating its performances on problems featuring nonlinear PDEs, singularities, and parametrized geometries.

==> design.tex <==
\subsection{Architecture design}
Having to deal with remarkably large dimensions, from $p$ to $\fomdim\times n$, the construction of a DOD architecture necessitates some discussion. As for other deep learning approaches, such as DL-ROM \cite{franco2023deep}, the complexity of this task can be decoupled in two parts. The first one, concerns the development of a suitable computational unit that process the input parameters, here given by $\mub\in\mathbb{R}^{p}.$ The second one, instead, involves the design of a proper terminal block that can tackle the high dimension at output. 

Taking these factors into account, we propose to design DODs according to the following scheme (see also Figure \ref{fig:dod} for a visual representation). The idea is to split the architecture in three parts:
\begin{itemize}
    \item[i)] a \textit{seed} module, given by a (dense) neural network $s:\mathbb{R}^{p}\to\mathbb{R}^{l}$, whose purpose is to pre-process the input parameters by mapping them onto a suitable feature space;
    \item[ii)] a \textit{root} module, comprised of $n$ stacked architectures, $R_{1},\dots,R_{n}$, each going from the feature space, $\mathbb{R}^{l}$, onto the high-fidelity space, $\mathbb{R}^{\fomdim}$, whose purpose is to compute the several columns of the DOD projector.
    \item [iii)] a \textit{Gram-Schmidt layer}, that is, a nonlearnable transformation that ensures $\mass$-orthonormality of the final output. We denote its action as
    $$\tilde{\mathbb{A}}\mapsto\mathbb{A}:=\text{Gram-Schmidt}(\tilde{\mathbb{A}},\;\text{inner} = \mass).$$
    By relying on the classical Gram-Schmidt procedure, the latter accepts any matrix $\tilde{\mathbb{A}}\in\mathbb{R}^{N_{h}\times n}$ and produces a corresponding $\mathbb{A}\in\mathbb{R}^{\fomdim\times n}$ such that $\spann(\mathbb{A})=\spann(\tilde{\mathbb{A}})$ and $\mathbb{A}^{T}\mass\mathbb{A}=\mathbb{I}$, with $\mathbb{I}\in\mathbb{R}^{n\times n}$ the identity matrix. 
\end{itemize}
Given an input parameter $\mub\in\pgeo\subset\mathbb{R}^{\ngeo}$, the corresponding DOD matrix at output is computed as
$$\dod_{\mub}:=\text{Gram-Schmidt}(\tilde{\dod}_{\mub},\;\text{inner} = \mass)\in\mathbb{R}^{\fomdim\times n},$$
where
$$\tilde{\dod}_{\mub}:=\left[R_{1}(s_{\mub}),\dots,R_{n}(s_{\mub})\right]\in\mathbb{R}^{\fomdim\times n},$$
and $s_{\mub}:=s(\mub).$ The idea is that $s$ acts as a "shared" reparametrization of the input, while the roots $R_{1},\dots,R_{n}$ operate independently to retrieve the (unorthonormalized) DOD basis. 

In general, assuming $\ngeo+l\ll\fomdim$, the seed module, $s$, can be constructed using classical dense architectures. Conversely, the roots $R_{1},\dots, R_{n}$ should be designed in terms of suitable layer types that can handle high dimensional data, such as, convolutional models (CNNs) or graph neural networks (GNNs). Here, we shall rely on mesh-informed neural networks (MINNs) \cite{franco2023mesh}, a new class of sparse architectures that was specifically designed to tackle mesh-based functional data, that is, to address those situations in which the high dimensions arise from the introduction of a Finite Element discretization. For further details about these architectures and their practical implementation, we refer to \cite{franco2023mesh}.

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{dod-sketch.pdf}
    \caption{Caption}
    \label{fig:dod}
\end{figure}

==> grassmann-training-algorithm.tex <==
\begin{algorithm}
\SetAlgoLined
\normalem
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\vspace{0.25em}
\Input{FOM solver $\texttt{FOM}=\texttt{FOM}(\mub,\nub)$, parameter spaces $\pgeo$ and $\pphys,$ DOD architecture class $\mathscr{D}$, basis dimension $n$, sample size $\ntrain$, local sample size $k$.
\vspace{0.25em}
}

\Output{Trained DOD model $\dod_{*}$.
\vspace{0.75em}
}

 $[\mub_{1},\dots,\mub_{\ntrain}]\leftarrow$ i.i.d. random sample from $\pgeo$\vspace{0.5em}

 $\mathbf{L}\leftarrow[\;]$ empty list\vspace{0.5em}

\For{\textnormal{$i = 1,\dots,\ntrain$}}{\vspace{0.25em}
$[\nub_{1},\dots,\nub_{k}]\leftarrow$ i.i.d. random sample from $\pphys$\vspace{0.25em}\\
$[\ub_{1},\dots,\ub_{k}]\leftarrow[\texttt{FOM}(\mub_{i},\nub_{j})\;\text{for}\;j=1,\dots,k]$\vspace{0.25em}\\
$\mathbf{L}\leftarrow[\mathbf{L},\;\texttt{POD}_{n}(\{\ub_{1},\dots,\ub_{k}\})]$\vspace{0.25em}
}
\vspace{0.25em}
$[\mathbb{V}_{1},\dots,\mathbb{V}_{\ntrain}]\leftarrow\mathbf{L}$\vspace{0.5em}

$\dod_{*}\leftarrow\argmin_{\dod\in\mathscr{D}}\;\frac{1}{\ntrain}\sum_{i=1}^{\ntrain}\distance_{s}(\mathbb{V}_{i},\;\dod(\mub_{i}))^{2}$\vspace{0.5em}

\Return{$\dod_{*}$}\vspace{0.25em}

 \caption{\label{algo:train2}Training of a DOD architecture (Grassmann manifold version, Section \ref{subsubsec:grassmann}). Here, $\distance_{s}(\mathbb{A},\mathbb{B}):=\distance(\spann(\mathbb{A}),\spann(\mathbb{B}))$, computed as in Algorithm \ref{algo:distance}. \vspace{0.25em}}
 
\end{algorithm}
